DDPG Learning for Aerial RIS-Assisted MU-MISO Communications

This paper defines the problem of optimizing the downlink multi-user multiple input, single output (MU-MISO) sum-rate for ground users served by an aerial reconfigurable intelligent surface (ARIS) that acts as a relay to the terrestrial base station. The deep deterministic policy gradient (DDPG) is proposed to calculate the optimal active beamforming matrix at the base station and the phase shifts of the reflecting elements at the ARIS to maximize the data rate. Simulation results show the superiority of the proposed scheme when compared to deep Q-learning (DQL) and baseline approaches.

==> include/related.tex <==
\textcolor{red}{It is good practice to have a separate section. Where space is limited, it can be included in the intro or other parts. Also we need to compare our results and conclusions to those from recent related works, those that apply, later in the paper.}

==> include/result2.tex <==
In this section, we analyze the performance of the proposed DQN-based UAV positioning and power control scheme in this paper for optimizing the secrecy capacity of the ground legitimate user in the presence of an eavesdropping attack. 

The simulation scenario consists of a single antenna ground UE, ABS mounted on an the UAV, and a single antenna malicious node that is performing a passive eavesdropping attack on the UL transmission initiated at the UE towards the ABS. The simulation scenario is shown in Fig.~\ref{fig:system}. The UE and the eavesdropper will be randomly distributed within a 2D area that has a $L_x$ length and a $L_y$ width. The ABS will be launched at random location with a fixed altitude and equipped with an omnidirectional antenna to facilitate the communication links with the served ground users. 

The simulation parameter and the hyperparameters for the proposed DQN solution are given in Table.~\ref{tab:parameters}. In particular, the training and target DNN networks consist of $4$ \hl{Why 4?} layers where each DNN contains two fully connected \hl{hidden} layers with $24$ and $32$ neurons, respectively. Each DNN has $3$ neurons at the input layer and $12$ neurons at the output layer, corresponding to the number of states \hl{(3)} and possible actions \hl{(12)}. \textcolor{red}{Have you explained what those states and actions are?}
The simulator %environment described in this paper is simulated in the 
is implemented in Python, using the PyTorch to train a DQN. %, while the illustration of the results has been performed using Matlab. 

In the evaluation of the performance of our proposed DQN algorithm, we are comparing the obtained secrecy capacity via the DQN against the same metric resultant from employing the Q-learning, greedy policy, and randomized states algorithms. 
The random scheme select the next position and power action at each time slot randomly, whereas the greedy policy assign the next action based on the highest Q-value \hl{continuously}. 
\begin{table}[t]
%\fontsize{12}{10}\selectfont
\fontsize{4}{8}\selectfont
\centering
\caption{Simulation parameters.}
\label{tab:parameters}
\resizebox{0.35\textwidth}{!}
{%
\begin{tabular}{|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Simulation  parameter}\end{tabular}     & \textbf{Value}                              \\ \hline
\begin{tabular}[c]{@{}c@{}}(L$_x$, L$_y$)\end{tabular} & (10, 10) m  \\ \hline
%\begin{tabular}[c]{@{}c@{}}L_y\end{tabular} & 10 m   \\ \hline
\begin{tabular}[c]{@{}c@{}} Number of episodes\end{tabular} & 9 $\times$ 10$^{4}$ \\ \hline
\begin{tabular}[c]{@{}c@{}} Number time slots per episode\end{tabular} &  200 \\ \hline
\begin{tabular}[c]{@{}c@{}} Learning rate\end{tabular} &  10$^{-6}$ \\ \hline
\begin{tabular}[c]{@{}c@{}} Discount factor\end{tabular} & 0.9 \\ \hline
%Noise variance                                                     & 10^{\text{-12} }       \\ \hline
%\begin{tabular}[c]{@{}c@{}}
%SNR at the reference point\end{tabular}                                                      & 90 dB       \\ \hline
%\begin{tabular}[c]{@{}c@{}}dx    \end{tabular}        & 20 m                               \\ \hline
%M                                                          & 5 users                              \\ \hline
%\begin{tabular}[c]{@{}c@{}} Number of DNN layers\end{tabular} & 4 \\ \hline
%\begin{tabular}[c]{@{}c@{}} Number of NN nodes\end{tabular} &  \\ \hline
\begin{tabular}[c]{@{}c@{}} Replay memory size\end{tabular} & 500 entries \\ \hline
\begin{tabular}[c]{@{}c@{}} Batch size\end{tabular} & 50 \\ \hline
\begin{tabular}[c]{@{}c@{}} Update rate of target network\end{tabular} & 10 \\ \hline
% Bandwidth                                                          & 10 MHz                              \\ \hline
\end{tabular}%
}
\vspace{-5mm}
\end{table}
    \begin{figure*}
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{{figures/Reward.eps}}
    \caption{The reward}
    \label{fig:Reward}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/Distance.eps}
    \caption{The distance}
    \label{fig:Distance}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/Power.eps}
    \caption{The power}
    \label{fig:PW}
  \end{subfigure}
  \caption{The reward, distance and power convergence of the DQN, Q-learning and other base line techniques.}\label{fig:animals}
\end{figure*}

 
Figure.~\ref{fig:Secrecy} illustrates the obtained secrecy capacity for the DQN compared to the other %benchmarking 
techniques over the number of episodes. %AS it can be noted, 
The proposed DQN algorithm enhances the episode secrecy capacity by as much as 40\%, 10\%, and 5\% when compared to the randomized states, greedy policy, and the Q-learning, respectively. According to Figure.~\ref{fig:Secrecy}, the performance of the DQN reaches a relatively stable secrecy capacity value after $1 \times 10^4$ episodes. On the other hand, the convergence of Q-learning occurs after $5 \times 10^4$ episodes. This proves the superiority of the DQN regarding the speed of convergence. %\hl{explain why accepted or remove rest of the sentence:} with accepted secrecy capacity performance over the other techniques.
%   \begin{figure}[H]
%      \centering
%      \includegraphics[width=0.45\textwidth]{figures/Secrecy.eps}
%      \caption{Secrecy.}
%      %\vspace{-5mm}
%      \label{fig:Secrecy}
%  \end{figure}

Since the secrecy capacity optimization problem relies on the location of the ABS and the transmission power, it is critical to study the convergence of these two parameters for a better understanding of the secrecy capacity performance. Figures~\ref{fig:Distance} and~\ref{fig:PW} illustrate the convergence of the UAV positioning and the transmission power over the number of episodes, respectively. Comparing the converged position of the ABS and transmission power for the DQN and Q-learning, we can see that both techniques have reached the same ABS position, however there is a slight increase of the converged transmission power of the DQN over the converged Q-learning transmission power. This difference %in the converged transmission power 
is the main explanation behind the difference in the obtained secrecy capacity levels presented in Fig.~\ref{fig:Secrecy}. Moreover, the zero secrecy capacity of the randomized states approach %given that both of the greedy and random approaches have converged to the same position from Fig.~\ref{fig:Distance} is resultant 
results from low transmission power value shown in Fig.~\ref{fig:PW}. Note that the ABS position converges to the same as with the greedy algorithm.

%   \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.45\textwidth]{figures/Distance.eps}
%      \caption{Distance.}
%      %\vspace{-5mm}
%      \label{fig:Distance}
%  \end{figure}
%  \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.45\textwidth]{figures/Power.eps}
%      \caption{Power.}
%      %\vspace{-5mm}
%      \label{fig:PW}
%  \end{figure}
%   \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.45\textwidth]{figures/Reward.eps}
%      \caption{Reward.}
%      %\vspace{-5mm}
%      \label{fig:Reward}
%  \end{figure}
Figure.~\ref{fig:Reward} shows our reward function that is defined as the legitimate UL capacity between the ground UE and the ABS without taking into consideration the eavesdropping capacity for the proposed DQN and other techniques. The illustrated reward functions inform that the proposed solution in this paper has the fastest convergence rate with higher capacity. On the other hand, the performance of the Q-learning is sufficient, but takes longer to converge because of the nature of the problem that has a large number of states. 
%  \begin{figure*}
%         \centering
%         \begin{subfigure}[b]{0.33\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{figures/Secrecy.eps}
%             \caption[Network2]%
%             {{\small Network 1}}    
%             \label{fig:mean and std of net14}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.33\textwidth}  
%             \centering 
%             \includegraphics[width=\textwidth]{figures/Distance.eps}
%             \caption[]%
%             {{\small Network 2}}    
%             \label{fig:mean and std of net24}
%         \end{subfigure}
%         \vskip\baselineskip
%         \begin{subfigure}[b]{0.33\textwidth}   
%             \centering 
%             \includegraphics[width=\textwidth]{figures/Power.eps}
%             \caption[]%
%             {{\small Network 3}}    
%             \label{fig:mean and std of net34}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.33\textwidth}   
%             \centering 
%             \includegraphics[width=\textwidth]{figures/Reward.eps}
%             \caption[]%
%             {{\small Network 4}}    
%             \label{fig:mean and std of net44}
%         \end{subfigure}
%         \caption[ The average and standard deviation of critical parameters ]
%         {\small The average and standard deviation of critical parameters: Region R4} 
%         \label{fig:mean and std of nets}
%     \end{figure*}
    
\begin{figure}[H]
     \centering
     \includegraphics[width=0.35\textwidth]{figures/Secrecy.eps}
     \caption{Secrecy.}
     %\vspace{-5mm}
     \label{fig:Secrecy}
 \end{figure}

==> include/system.tex <==
The scenario %of interest that we considered
%that is 
studied in this paper is illustrated in~Fig.~\ref{fig:system}. The ground user communicates with the ABS %provided by the aerial node 
in the presence of a terrestrial eavesdropper.  
The user and eavesdropper are independent of each other. % randomly distributed within a predefined grid dimension. 
The ABS is positioned to provide a secure and reliable uplink (UL) %communication %traffic 
for the user under attack. It achieves this by leveraging its 3D mobility and strong line of sight (LoS) channel that allows low power transmission. %links over the terrestrial communication links supplied by the terrestrial base stations. 
Without loss of generality, we model and analyze the UL channel here. The same principles can be applied for the downlink (DL).
In the rest of this paper, we use the UAV and ABS interchangeably. %, but they convey the same meaning.
 \begin{figure}[t]
 \vspace{-1mm}
     \centering
     \includegraphics[width=0.40\textwidth]{figures/SystemModel_DQLUAV.eps}
     \vspace{-1mm}
     \caption{The simulation scenario.}
     \vspace{-6mm}
         \label{fig:system}
 \end{figure}
%The set of $M$ users in the cluster %being attacked 
%and the set of $K$ eavesdroppers are denoted as $V=\{V_i|i=1,2,...,M\}$ and $E=\{{E}_{j}|j=1,2,...K\}$, respectively.
%Without loss of generality, 

We define the location of the ABS, the eavesdropper, and the user in the 3D Cartesian coordinate system as ($x_u,y_u,z_u$), ($x_j,y_j,z_j$), and ($x,y,z$), respectively.
%%The UAV flies at the % has a fixed 
%%altitude $z_u$, which may be chosen according to %considered as
%%the minimum height at which the UAV will have line of sight (LoS) links with the users in the cluster%, and where it would avoid buildings and obstacles from the air
%%~\cite{UAVLoS}. 
%%The UAV relay operation %along the cluster travel distance
%%will be executed over a finite duration $T$. 
For practicality, %we distribute the UAV relaying period over $N$ 
time slots are used to capture the different radio frames and statistical channel conditions, as well as the momentarily static position of the nodes. %ABS, users, and eavesdroppers. %, equally. 
Therefore, the ABS coordinates in time slot $t$ are expressed as ($x_u[t], y_u[t], z_u[t]$).    

\subsection{Communications Channel} 
The received signal at the ABS when the ground user equipment (UE) %initiate the transmission process for 
transmits the signal $s$ with power $P$ is as follows
%\vspace{-1 mm}
\begin{equation}
    {r} = \sqrt{P\hbar}s+n,
 %  \vspace{-2 mm}
\end{equation}
where $\hbar$ is %corresponding to 
the air-to-ground (A2G) channel %power 
gain between the UE and the ABS, and $n$ denotes the additive white Gaussian noise (AWGN) of zero mean and $\sigma^2$ variance. %
Based on the measurements presented in~\cite{R4}, %we can assume that 
the LoS %channel 
model is a good approximation for the A2G channel in rural areas. %, specifically when the UAV flies at higher altitudes.% 80 m.  
The channel gain %${g}_{iu}[n]$ 
%in time slot $n$ 
has %is characterized by
a path loss exponent of two and can be written as
%\vspace{-1 mm}
\begin{equation}
\small
\begin{aligned}
    \hbar[t] &=\zeta_{0}d^{-2}_{u}[t] \\
    &=\frac{\zeta_0}{(x[t]-x_u[t])^2+(y[t]-y_u[t])^2+(z[t]-z_u[t])^2},
    \end{aligned}
    \label{eq:channel_gain1}
\end{equation}
where $\zeta_{0}$ is the channel gain at the reference point $d_0$ = 1 m. Parameter $\zeta_{0}$ is the same for the A2G and the ground-to-ground (G2G) channel %model and will not be differentiate due to 
because of the same the antenna gains and carrier frequency in both cases. Parameter $d_{u}[t]$ denotes the distance between the ground user and the ABS. 

The capacity of the channel between the UE and the ABS in time slot $t$ is calculated as follows: 
%\vspace{-1 mm}
\begin{equation}
%\small
%\begin{aligned}
    {C _{u}[t]} = \log_2 \left( 1+\frac{{P}[t]\hbar[t]}{\sigma^2}\right) = \log_2 \left( 1+\frac{\zeta_0{P}[t]}{d^2_{u}[t]\sigma^2}\right),
    %{(x_i[n]-x_u[n])^2+(y_i[n]-y_u[n])^2[n]+(z_i[n]-H)^2}
%\end{aligned}
\label{eq:cap_UAV-UE}
\end{equation}
where $\zeta_0/\sigma^2$ is the signal-to-noise ratio (SNR) at the reference point. 

\subsection{Eavesdropping Channel} %{Because the UAV is in the air and can often establish an LoS link with the BS, beamforming and PC can be effectively employed to focus the radio frequency (RF) transmission between the BS and UAV. %and reduce the radiated energy. 
%The restricted space and size of the ground users such as the small Internet of things (IoT) devices and sensors, smartphones and portable devices enforce the use of single or fewer transmit antenna per each user, 
Often, UEs have fewer antennas %which is commonly 
and transmit in broadcast mode without beamforming. % or directed behavior. Therefore, the UL links will not be focused and can be easily comprised. %Assuming ground eavesdroppers, here we therefore consider the user-UAV link being the dominant eavesdropping channel.
The eavesdropper is intercepting the transmitted signal from the ground UE and the received signal can be formulated as
%\vspace{-2 mm}
\begin{equation}
    {v } = \sqrt{P{\emptyset}}s+w,
%    \vspace{-2 mm}
\end{equation}
where $w$ denotes the zero-mean 
AWGN with a variance of $\sigma^2$ 
at the eavesdropper. 
As a result of the G2G communications link between the UE and the eavesdroppers, the exponent of the path loss for this link is assumed to be four. Within the time slot $t$, the G2G channel %power 
gain represented by $\emptyset$ between the UE and eavesdropper can be modeled as
\vspace{-0.5 mm}
\begin{equation}
\small
\begin{aligned}
    %{w}_{ij}[n] &=\omega_{0}d^{-4}_{ij}[n]\\
    %=&\frac{\omega_0}{({(x_i[n]-x_j[n])^2+(y_i[n]-y_j[n])^2+(z_i[n]-z_j[n])^2)}^2},
    \emptyset &=\zeta_{0}d^{-4}_{j}[t]\\
    =&\frac{\zeta_0}{({(x[t]-x_j[t])^2+(y[t]-y_j[t])^2+(z[t]-z_j[t])^2)}^2},
    \end{aligned}
\end{equation}
where $d_{j}[t]$ corresponds to the distance between the %transmitter 
UE and the eavesdropper in the $t$th time slot.
The corresponding capacity of the wiretap channel is 
%\vspace{-2 mm}
\begin{equation}
%\small
%\begin{aligned}
    {C _{j}[t]} = \log_2 \left( 1+\frac{{P}[t]{\emptyset}[t]}{\sigma^2}\right) = \log_2 \left(
    1+\frac{\zeta_{0}{P}[t]}{d^{4}_{j}[t]\sigma^2}\right).
    %1+\frac{\delta_0{P_i}[n]}{d^{4}_{ij}[n]})\right),
    %(x_i[n]-x_j[n])^2+(y_i[n]-y_j[n])^2[n]+(z_i[n]-z_j[n])^2
 %   \end{aligned}
\end{equation}
%where $\delta_0=\omega__0/\sigma^2$ is the signal-to-noise ratio(SNR) at the reference point. 
%This work considers the case of uncoordinated eavesdropping attacks. 
%between the available eavesdroppers. 
%%Therefore, if the transmission between the BS and $V_i$ has been interpreted successfully by any eavesdropper, the transmission will be exposed to other attackers. 
%As a result of that, 
%\textcolor{blue}{ We assume that the UE-AR links are subject to eavesdropping, whereas the BS-AR link can be more focused and is therefore less susceptible to eavesdropping.}
% As a result, the capacity of the eavesdropping channel is calculated as the maximum %achieved 
% capacity among the $K$ eavesdroppers:
% \vspace{-2.5 mm}
% \begin{equation}
%     {C _{ij}[n]} = \max\limits_{j \in E} C _{ij}[n] = \max\limits_{j \in E} \log_2
%     \left( 1+\frac{\lambda_0{P_i}[n]}{d^{4}_{ij}[n]}\right).
%     %\left( 1+\frac{\delta_0{P_i}[n]}{d^{4}_{ij}[n]}\right),
% \end{equation}
% \vspace{-10mm}
\subsection{Secrecy Capacity Metric}
The security of the system is evaluated using the secrecy capacity metric which is %a common metric that has been 
commonly employed in the literature for analyzing %various
eavesdropping security problems. %in cellular networks.   
The secrecy capacity is the rate at which the malicious node cannot decode any %further 
data %positive divergence level that occurs 
when the legitimate channel capacity is higher than the wiretap channel capacity~\cite{YanWanGer2015}. %  which is associate to the rate at which no data will be decoded by the eavesdropper~\cite{YanWanGer2015}.  
The secrecy capacity over $T$ %radio 
time slots %with a scenario consisting of a ground eavesdropper, UE, and ABS
is then obtained as
%\vspace{-2 mm}
\begin{equation}
    {C_{sec}} = \frac{1}{T}\sum\limits_{t=1}^T \bigg(
    C_{u}[t]- C_{j}[t] \bigg)^+,
    \label{equ:totalsec}
\end{equation}
%\vspace{4 mm}
where $[\omega]^+ \triangleq max(\omega,0)$.% returns the maximum value between the provided $\omega$ and the null value.

\subsection{Problem Formulation }%\hl{independent section?}}
The optimization problem %in~(\ref{eq:opt_secrecy_rate}) 
is defined 
according to the following %number of 
assumptions: 
%in order to ensure the efficiency of the proposed solution described in the next section. 
First, for the sake of simplicity and without loss of generality, we assume that an ABS flies at a constant height that %. This 
facilitates a LoS link between the ABS and the ground UE. In general, the lower the UAV height can be, the higher the resulting legitimate channel and secrecy capacity in the considered context. Second, we assume that the location of the passive eavesdropper is unknown. % in the problem.
This scenario is of interest in practice where it is difficult to detect the presence and location of eavesdroppers because of their passive nature. % is difficult. 
Thus, we consider the capacity of the legitimate user in the above problem formulation. % in~(\ref{eq:opt_secrecy_rate}). 
The eavesdropper location is used only for the calculation of the resulting secrecy rate to evaluate the performance of the proposed solution. % \hl{we may remove the last part 'to evaluate...' because are we evaluating it against some known benchmark, e.g. reported secrecy rates in literature, or are all considered algorithms unaware of the eavesdropper's location}.

The objective of this paper is thus to maximize the legitimate capacity $C_{u}$  
by selecting the %optimal 
position for the ABS and controlling transmit power %allocation 
for the UE.   
%performing optimal transmission power policy. 

The optimization of the UE capacity will result in an improved secrecy capacity of the system. %under passive eavesdropping. %is relying on enhancing the UL capacity of the legitimate UE.
However, the UL capacity of the ground user relies on having a short distance to the ABS  
with a strong LoS link. % with the effected UEs. 
Therefore, the ABS position constraint is formulated as follows:
\begin{equation}
    (x_u[t],y_u[t]) \leq (L_x,L_y), \forall {t},
\end{equation}
where $(L_x,L_y)$ represent the maximum 2D coordinates of the UAV ground location projection. %area where the simulation scenario is performed. 
We introduce the peak transmission power $ P_{max}$ and the UL transmission power constraint for the legitimate UE per time slot as  
\begin{equation}
   0 \leq P[t] \leq P_{max}, \forall {t}.
   \label{11}
\end{equation}
The optimization problem of the UE capacity %$C_{u}$ %can now be written as
is then given as
\begin{equation}
\begin{aligned}
   (P1) : \max\limits_{x_u,y_u,P} \frac{1}{T}\sum\limits_{t=1}^T \Bigg[ %\frac{1}{M}
     &\log_2 \left( 1+\frac{\zeta_0{P}[t]}{d^2_{u}[t]\sigma^2}\right)%\\
   %- &\log_2 \left( 1+\frac{\zeta_{0}{P}[t]}{d^{4}_{j}[t]\sigma^2}\right) 
   \Bigg]%^+
   ,\\
   s.t.\hspace{2 pt }(8),(9).
   \end{aligned}
   \label{eq:opt_secrecy_rate}
\end{equation}
%\textcolor{black}{\textbf{Assumptions:}} %List the assumptions that you make or not make as this may be the distinguishing factor or this work w.r.t. others. Justify your assumptions.}
%The following proposed solution for
where $x_u$ and $y_u$ are the UAV positioning parameters and $P$ is the uplink transmission power controlled by the ABS. %for the UAV positioning and the uplink power control of the UE. % which is controlled by the ABS.




==> include/systemEXCLUDED.tex <==
Denote the transmitted data symbol to the $k^{th}$ GT by $s_k$, which is independent random variable with zero mean and unit variance. Then, the transmitted signal at the GBS can be defined as follow 
\begin{equation}
        v =   \sum\limits_{k=1}^K \vb*{w_k} \ s_k, 
    \label{eq:xs}, 
\end{equation}
where $\vb*{w}_{k} \in\mathbb{C}^{M \times 1}$ is the beamforming vector of the $k^{th}$ GT applied at the GBs. The beamforming matrix of the BS (a.k.a. precoding matrix) contains $K$ beamforming vectors, denoted by $\vb*{W} \in \mathbb{C}^{M \times K}$, where $\vb*{W} =[\vb*{w}_{1}, \cdots, \vb*{w}_{K}]$. The allocated transmit power for the $k^{th}$ GT can then be calculated by the squared norm of the beamforming vector $\parallel\vb*{w}_{k} \parallel^2$. The received signal at the ARIS node can be expressed as 
% \begin{align}\label{eq:relay_1}
% \notag   \vb*{y}_{R} &= \vb*{G}_{TR} \ \vb*{v} + \vb*{n}_{1},\\
%                      &= \vb*{G}_{TR} \Big( \sum\limits_{k=1}^K \vb*{w}_{k} \ s_k \Big) + \, \vb*{n}_R,
% \end{align}
\begin{align}\label{eq:relay_1}
\notag   \vb*{y}_{R} &= \vb*{G}_{TR} \ \vb*{v} ,\\
                     &= \vb*{G}_{TR} \sum\limits_{k=1}^K \vb*{w}_{k} \ s_k ,
\end{align}
%where $\vb*{n}_R \in \mathbb{C}^{N\times 1}$ is the noise vector at the ARIS such that $\vb*{n}_1 \sim \mathcal{CN}(0, \vb*{I})$.
It is worth noting that the passive property of the reflecting elements employed in the RIS-based wireless communications provides an efficient end-to-end communication performance by only reflecting the arriving signals without decoding and, therefore it prohibit the injection of AWGN in the reflected path. After receiving $\vb*{y}_{R}$ at the ARIS, the ARIS starts preparing $\vb*{x}_{R}$ to be transmitted towards the $K$ UEs with the phase shifts matrix $\vb*{\phi} \in \mathbb{C}^{N\times N}$. Thus, the transmission signal at the ARIS, $\vb*{x}_r$ is given as follow
% \begin{align}\label{eq:relay_2}
% \notag        \vb*{x}_R &= \vb*{\phi} \ \vb*{y}_{R},\\
%                         &=\vb*{\phi} \bigg( \vb*{G}_{TR} \Big( \sum\limits_{k=1}^K \vb*{w}_{k} \ s_k \Big) + \vb*{n}_R \bigg)
% \end{align}
\begin{align}\label{eq:relay_2}
\notag        \vb*{x}_R &= \vb*{\phi} \ \vb*{y}_{R},\\
                        &=\vb*{\phi} \bigg( \vb*{G}_{TR} \Big( \sum\limits_{k=1}^K \vb*{w}_{k} \ s_k \Big) \bigg)
\end{align}
% Hence, the received signal at the $K$ UEs from the AR, $\vb*{y}_2 \in \mathbb{C}^{K\times 1}$, can be written as 
% \begin{align}\label{eq:relay_3}
% \notag        \vb*{y}_2 &= \vb*{H}_2 \ \vb*{x}_r + \vb*{n}_2,\\
%                         &= \vb*{H}_2 \, \Bigg( \vb*{W}_r \, \bigg( \vb*{H}_1 \Big( \sum\limits_{k=1}^K \vb*{w}_{b,k} \ s_k \Big) + \, \vb*{n}_1   \bigg)  \Bigg) + \vb*{n}_2,
% \end{align}
% where $\vb*{H}_2 \in \mathbb{C}^{K\times N}$ is the A2G communication channel between the AR and the $K$ UEs, and $\vb*{n}_2 \in \mathbb{C}^{K\times 1}$ is the noise vector at the $K$ UEs such that $\vb*{n}_2 \sim \mathcal{CN}(0, \vb*{I})$.
Hence, the received signal at the $k^{th}$ GT from the ARIS can be written as 
% \begin{align}\label{eq:relay_4}
% \notag         y_{Rk} &= \vb*{g}_{Rk} \vb*{\phi} \ \vb*{G}^{TR} \ \vb*{w}_{k} \ s_k  \\
% \notag                 & + \vb*{g}_{Rk} \vb*{\phi} \ \vb*{G}^{TR}  \Big( \sum\limits_{i\neq k}^K \vb*{w}_{i} \ s_i \Big)\\ 
%                         & +  \vb*{g}_{Rk} \vb*{\phi} \ \vb*{n}_R + n_{k},
% \end{align}
\begin{align}\label{eq:relay_4}
\notag         y_{Rk} &= \vb*{g}_{Rk} \vb*{\phi} \ \vb*{G}^{TR} \ \vb*{w}_{k} \ s_k  \\
\notag                 & + \vb*{g}_{Rk} \vb*{\phi} \ \vb*{G}^{TR}  \Big( \sum\limits_{i\neq k}^K \vb*{w}_{i} \ s_i \Big) +  n_{k},
\end{align}
where $\vb*{g}_{Rk} \in \mathbb{C}^{1\times N}$ denotes the channel vector from the ARIS to the $k^{th}$ GT, and $n_{k}$ is the noise at the $k^{th}$ GT such that $n_{k}\sim \mathcal{CN}(0, 1)$. The second term in the formula of the $y_{RK}$ is corresponding to the interference produced from the transmission of other GTs om the $k^{th}$ GT signal, this interference is commonly known as multi-user interference. By taken into consideration the multi-user interference, the signal-to-interference ratio (SINR) at the $k^{th}$ GT is denoted as 
% \begin{equation}
%         \vb*{\gamma}_{k} =   \frac{\mid \vb*{g}_{Rk} \vb*{\phi} \ \vb*{G}^{TR} \ \vb*{w}_{k} \mid^2}{\sum\limits_{i\neq k}^K \mid \vb*{g}_{Rk} \vb*{\phi} \ \vb*{G}^{TR} \vb*{w}_{i} \mid^2 + \mid \vb*{g}_{Rk} \vb*{\phi} \mid^2 \sigma^2_R + \sigma^2_{k}}, 
%     \label{eq:xs}, 
% \end{equation}
\begin{equation}
        \vb*{\gamma}_{k} =   \frac{\mid \vb*{g}_{Rk} \vb*{\phi} \ \vb*{G}^{TR} \ \vb*{w}_{k} \mid^2}{\sum\limits_{i\neq k}^K \mid \vb*{g}_{Rk} \vb*{\phi} \ \vb*{G}^{TR} \vb*{w}_{i} \mid^2 +  \sigma^2_{k}} 
    \label{eq:xs}, 
\end{equation}
where $\sigma^2_{k}$ is the variance of noise at the $k^{th}$ GT, $\vb*{w}_{k} \in\mathbb{C}^{M \times 1}$ is the beamforming vector of the $k^{th}$ GT applied at the GBs. The GBS beamforming matrix contains $K$ beamforming vectors, denoted by $\vb*{W} \in \mathbb{C}^{M \times K}$, where $\vb*{W} =[\vb*{w}_{1}, \cdots, \vb*{w}_{K}]$. The allocated transmit power for the $k^{th}$ GT can then be calculated by $\parallel\vb*{w}_{k} \parallel^2$.
Thus, the achieved sum-rate of the system can be calculated as follows
\begin{equation}
        \vb*{\rho} =   \sum\limits_{k=1}^K log_2 \ (1+\vb*{\gamma}_{k})
    \label{eq:xs}, 
\end{equation}
